Similarity Learning with Higher-Order Graph Convolutions for Brain Network Analysis

Learning a similarity metric has gained much attention recently, where the goal is to learn a function that maps input patterns to a target space while preserving the semantic distance in the input space. While most related work focused on images, we focus instead on learning a similarity metric for neuroimages, such as fMRI and DTI images. We propose an end-to-end similarity learning framework called Higher-order Siamese GCN for multi-subject fMRI data analysis. The proposed framework learns the brain network representations via a supervised metric-based approach with siamese neural networks using two graph convolutional networks as the twin networks. Our proposed framework performs higher-order convolutions by incorporating higher-order proximity in graph convolutional networks to characterize and learn the community structure in brain connectivity networks. To the best of our knowledge, this is the first community-preserving similarity learning framework for multi-subject brain network analysis. Experimental results on four real fMRI datasets demonstrate the potential use cases of the proposed framework for multi-subject brain analysis in health and neuropsychiatric disorders. Our proposed approach achieves an average AUC gain of 75% compared to PCA, an average AUC gain of 65.5% compared to Spectral Embedding, and an average AUC gain of 24.3% compared to S-GCN across the four datasets, indicating promising application in clinical investigation and brain disease diagnosis.

==> sec-framework.tex <==
\section{Similarity Learning Framework for Multi-Subject fMRI Data}
\label{sec:framework}
%\textbf{\textcolor{red}{Nesreen: should we move this paragraph to the related work and merge it there?

%\textbf{\textcolor{blue}{Nesreen: Add a few sentences about the the multi-subject fMRI data and applications}}

% \textbf{\textcolor{blue}{Nesreen: Formalize the multi-subject problem (e.g., Given a data set ...), and make sure everything flows}}

% \textbf{\textcolor{blue}{Nesreen: Clean up and shrink the discussion on GCN, and algorithm description. make it to the point, and make sure everything is formalized}}

%In many neuroscience study, fMRI brain data are usually acquired for a group of subjects under the same condition and environment. These fMRI data reflect the functional activity patterns of multiple subjects and thus are very important for the multi-subject analysis such as the group-contrasting pattern analysis for brain disorder diagnosis \cite{chen2011quantitative} or cognitive analysis \cite{dubois2018distributed}. Therefore, measuring similarity between the fMRI brain networks of different subjects is especially important for those further analysis like brain disorder diagnosis. 

% Given a multi-subject fMRI data set $D = \{G_1,G_2,\cdots ,G_N\}$ where $G_i$ is the fMRI brain network of subject $i$, the goal of similarity learning for the multi-subject fMRI data is to learn a model with optimal parameter weights $\mathbb{W}$ that maps the brain networks to a target space, such that the loss function is small if the input pairs $(G_1, G_2)$ belonging to the same class, and large if the input pairs $(G_1, G_2)$ belonging to different classes. The loss function used in training maximizes the mean similarity between input pairs belonging to the same class, and minimizes the mean similarity between pairs belonging to different classes. 
%\vspace{-1mm}
%\paragraph{\textbf{Problem Definition.}}
\begin{figure*}[t]
\centering
    \begin{minipage}[l]{0.7\linewidth}
      \centering
      \includegraphics[width=0.9\linewidth]{framework.png}
    \end{minipage}
  \caption{The Higher-order Siamese-GCN framework}\label{fig:framework}
  \vspace{-4mm}
\end{figure*}

We propose an end-to-end framework called \emph{higher-order Siamese GCN} for learning the similarity among fMRI brain connectivity networks extracted from multiple subjects. We assume each brain network is represented by a graph where the nodes represent brain regions and the edges represent the inter-regional associations. Our proposed framework (presented in Fig.~\ref{fig:framework}) consists of the following: (1) a Siamese neural network architecture, (2) two identical higher-order graph convolutional networks used as the twin network, (3) a dot product layer, and (4) a fully connected layer. 
%Siamese network has been shown to be an effective architecture for solving image matching problems such as signature verification \cite{{bromley1994signature}} and image recognition \cite{chopra2005learning}. 
The framework takes an input pair of graphs, such that each graph is processed by one branch of the siamese network (i.e., each graph is processed by one of the identical twin GCNs). Since the twin graph neural networks share the same weights, each input graphs is guaranteed to be processed in the same way by the twin networks respectively. As such, similar input graphs would be embedded similarly in the latent space. Our proposed framework performs higher-order convolutions by incorporating higher-order proximity using random walks in graph convolutional networks. Finally, the dot product layer combines the outputs from the two branches of the siamese network, then followed by a single fully connected (FC) layer with one output to estimate the similarity score.
%Therefore, the Siamese network is good for differentiating the two inputs or measuring the similarity between them. As shown in Fig.~\ref{fig:framework}, our Siamese framework takes two graphs as inputs, and a random walk procedure is applied on each of the graphs to obtain the higher-order proximity representations, which leads to the higher-order graph convolutions in each of the twin networks. A similarity estimate will be obtained based on the outputs of the twin higher-order GCNs. We employ the Hinge loss in Equation (\ref{hinge_loss}) for the training of the Siamese network. 

Given a multi-subject fMRI data set $\mathcal{G} = \{G_1,G_2,\cdots ,G_N\}$ where $G_i=(V_i, E_i, \mathbf{A_i})$ is the fMRI brain network of subject $i$, $V_i$ is the set of vertices in $G_i$, $E_i \subset V_i \times V_i $ is the set of edges in $G_i$, and $\mathbf{A_i} \in \mathbb{R}^{m \times m}$ is the affinity matrix of $G_i$, we assume that we have a model $\mathcal{M}$ with parameter weights $\mathbb{W}$ to map the brain networks to the feature/embedding space and the embedding of $G_i$ can be obtained as $H_i = \mathcal{M}(A_i)$. Assume we have a function $\mathcal{S}$ for computing similarity between the embeddings of two brain networks, and the similarity score between a pair of brain networks $G_i$ and $G_j$ is denoted by $s_{ij} = \mathcal{S}(H_i,H_j)$, the goal of similarity learning for the multi-subject fMRI data is to learn the optimal parameter weights $\mathbb{W}$ for $\mathcal{M}$ such that the value of $s_{ij}$ is large for an input pairs $(G_i, G_j)$ belonging to the same class, and small for input pairs $(G_i, G_j)$ belonging to different classes. The loss function used in training should maximize the mean similarity between input pairs belonging to the same class, and minimize the mean similarity between pairs belonging to different classes. 


% Assume we are given any pair of graphs $G_i=(V_i, E_i, \mathbf{A_i})$ and $G_j=(V_j, E_j, \mathbf{A_j})$ in a graph collection $\mathcal{G}$, where $V_i$ and $V_j$ are the sets of vertices with fully aligned physical meanings for $G_i$ and $G_j$ respectively. Let $\mathcal{M}$ be a function that predicts a similarity score $s$ between two input graphs $G_i$ and $G_j$, i.e., $s_{ij} = \mathcal{M}(G_i,G_j)$. Then $s_{ij} > s_{ik}$, if and only if $G_i$ is structurally similar to $G_j$ than to $G_k$, for any three graphs $G_i, G_j, G_k \in \mathcal{G}$.

%\textbf{Problem Definition.}
%Assume we are given a pair of graphs $G_i=(V_i, E_i, \mathbf{A_i})$ and $G_j=(V_j, E_j, \mathbf{A_j})$ in a graph collection $\mathcal{G}$, where $V_i$ and $V_j$ are the sets of vertices with fully aligned physical meanings for $G_i$ and $G_j$ respectively. The goal of similarity learning is to learn a model $\mathcal{M}$ that predicts the similarity score $s$ between $G_i$ and $G_j$, for any $G_i, G_j \in \mathcal{G}$. 
\vspace{-1mm}
\paragraph{\textbf{From fMRI data to brain connectivity networks.}}
% As shown in Figure~\ref{fig:brain}, a whole-brain fMRI image consists of a
A whole-brain fMRI image consists of a sequence of 3D brain image scans, where each volume consists of hundreds of thousands of voxels. Each voxel has an intensity value that is proportional to the strength of the Nuclear Magnetic Resonance (NMR) signal emitted at the corresponding location in the brain volume. The  raw form of an fMRI brain image is a discrete time series of 3D images. In order to convert the original fMRI images to region-by-region brain networks, we extract a sequence of responses from each of the regions of interest (ROI), where each ROI represents a brain region. We perform the standard fMRI brain image processing steps, including functional images realignment, slice timing correction and normalization, etc. Then, we compute the region-to-region brain activity correlations. We only keep the positive correlations as the links among the brain regions. The final constructed network is a graph where the nodes/vertices represent brain regions and the edges are the region-to-region correlations.

%We propose an end-to-end framework for learning the similarity among fMRI brain connectivity networks extracted from multiple subjects. We assume each brain network is represented by a graph where the nodes represent brain regions and the edges represent the correlations among them. Our framework is composed of a Siamese network with two higher-order graph convolutional networks as shown in Fig.~\ref{fig:framework}. Siamese network has been shown to be an effective architecture for solving image matching problems such as signature verification \cite{{bromley1994signature}} and image recognition \cite{chopra2005learning}. As the parameters between the twin neural networks in the Siamese network are shared, each input will be processed in the same way respectively in the twin networks, which can guarantee that similar input samples not be mapped to very different locations by the respective networks. Therefore, the Siamese network is good for differentiating the two inputs or measuring the similarity between them. As shown in Fig.~\ref{fig:framework}, our Siamese framework takes two graphs as inputs, and a random walk procedure is applied on each of the graphs to obtain the higher-order proximity representations, which leads to the higher-order graph convolutions in each of the twin networks. A similarity estimate will be obtained based on the outputs of the twin higher-order GCNs. We employ the Hinge loss in Equation (\ref{hinge_loss}) for the training of the Siamese network. 
%and the representation of each graph will be refined by a random walk procedure, which incorporates higher-order structural information into the graph representations and further enables the higher-order graph convolutions in each of the twin networks. 

 

%, making the similarity learning of these neuroimages a challenge problem. In this paper, we tackle this problem by looking at the brain connectivity networks derived from the original fMRI images and perform similarity learning on the brain networks, which will benefit various biomedical and cognitive neuroscience applications. 
%among different brain regions based on the obtained time series for each of them, and then we use the positive correlations as the links among the brain regions. Thus, each node in the constructed network represents a brain region, and the edge connecting two nodes represents the correlation between those two different brain regions. Then our goal is to learn a good representation for the fMRI brain network and leverage it in the similarity learning task.



\begin{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width = 0.45 \columnwidth]{Figure1_Siamese.png}
    \caption{Siamese Architecture with Graph Convolutional Networks}
    \label{fig:siamese}
\end{figure}
\end{comment}
\vspace{-1mm}
\paragraph{\textbf{Graph Convolutional Networks.}}
Graph convolutional network (GCN), as a generalized convolutional neural network from grid-structure domain to graph-structure domain, has been emerging as a powerful approach for graph mining \cite{bruna2013spectral,defferrard2016convolutional}. In GCNs, filters are defined in the graph spectral domain. In this paper, we employ the GCN with fast spectral filtering proposed in \cite{defferrard2016convolutional}. Given a graph $G=(V, E, \mathbf{A})$, where $V$ is the set of vertices, $E \subset V \times V $ is the set of edges, and  $\mathbf{A} \in \mathbb{R}^{m \times m}$ is the adjacency matrix, the diagonal degree matrix $\mathbf{D}$ will have elements $\mathbf{D}_{ii} = \sum_j \mathbf{A}_{ij}$. The graph Laplacian matrix is $\mathbf{L} = \mathbf{D} - \mathbf{A}$, which can be normalized as $\mathbf{L} = \mathbf{I}_m - \mathbf{D}^{-\frac{1}{2}}\mathbf{A} \mathbf{D}^{-\frac{1}{2}}$, where $\mathbf{I}_m$ is the identity matrix. Assume the orthonormal eigenvectors of $\mathbf{L}$ are represented as $\{u_l\}_{l=0}^{m-1}\in \mathbb{R}^{m \times m}$, and their associated eigenvalues are $\{\lambda_l\}_{l=0}^{m-1}$, the Laplacian is diagonalized by the Fourier basis $[u_0, \cdots,u_{m-1}](=\mathbf{U})\in \mathbb{R}^{m \times m}$ and $\mathbf{L} = \mathbf{U\Lambda U^T}$ where $\mathbf{\Lambda} = diag([\lambda_0,\cdots,\lambda_{m-1}])\in \mathbb{R}^{m\times m}$. The graph Fourier transform of a signal $x\in \mathbb{R}^m$ can then be defined as $\hat{x} = \mathbf{U^T}x \in \mathbb{R}^m$\cite{shuman2013emerging}. Suppose a signal vector $\mathbf{x} : V \rightarrow \mathbb{R}$ is defined on the nodes of graph $G$, where $\mathbf{x}_i$ is the value of $\mathbf{x}$ at the $i^{th}$ node. Then the signal $\mathbf{x}$ can be filtered by $g_\theta$ as

\begin{align}
    y = g_\theta*\mathbf{x} = g_\theta(\mathbf{L})\mathbf{x} = g_\theta(\mathbf{U{\Lambda}U^T})\mathbf{x} = \mathbf{U}g_\theta(\Lambda)\mathbf{U^T}\mathbf{x}
\label{eq:filter_signal}
\end{align}
where the filter $g_\theta(\Lambda)$ can be defined as $g_{\theta}(\Lambda) = \sum_{k=0}^{K-1}{\theta_k}{\Lambda^k}$, and the parameter $\theta\in {\mathbb{R}}^K$ is a vector of polynomial coefficients \cite{defferrard2016convolutional}. The above filter is exactly $K$-localized, which means the nodes with shortest path length greater than $K$ are not considered for the convolution. To further reduce computational complexity,  we use the Chebyshev polynomials \cite{defferrard2016convolutional} which can be computed recursively by $T_k(\mathbf{x}) = 2\mathbf{x}T_{k-1}(\mathbf{x}) - T_{k-2}(\mathbf{x})$ with $T_0 = 1$ and $T_1 = \mathbf{x}$, and a filter of order $K-1$ is parameterized as the truncated expansion 
\vspace{-2mm}
\begin{align}
    g_{\theta}(\Lambda) = \sum_{k=0}^{K-1}{\theta_k}T_k(\hat{\Lambda})
\end{align}
Then the filtering operation can be written as $y = g_\theta(\mathbf{L})\mathbf{x} = \sum_{k=0}^{K-1}\theta_kT_k(\hat{L})\mathbf{x}$, where $T_k(\hat{L})\in \mathbb{R}^{n\times n}$ is the Chebyshev polynomial of order $k$ with the Laplacian $\hat{L} = 2L/\lambda_{max} - I_n$. The $j^{th}$ output feature map of sample s is then given by
\vspace{-2mm}
\begin{align}
    y_{s,j} = \sum_{i=1}^{F_{in}}g\theta_{i,j}(L)x_{s,i}\in \mathbb{R}^m
\label{eq:filter}
\end{align}
where $x_{s,i}$ is the input feature map, and $F_{in}$ represents the number of input filters. The $F_{in}\times F_{out}$ vectors of Chebyshev coefficients $\theta_{i,j}\in \mathbb{R}^K$ are the layer's trainable parameters. Then we build the GCN by stacking multiple convolutional layers in the form of Equation (\ref{eq:filter}), with a non-linearity activation (ReLU) following each layer. 

% Graph convolutional network (GCN), as a generalized convolutional neural network from grid-structure domain to graph-structure domain, has been emerging as a powerful approach for graph mining \cite{bruna2013spectral,defferrard2016convolutional}. In GCNs, filters are defined in the graph spectral domain. Given a graph $G=(V, E, \mathbf{A})$, where $V$ is the set of vertices, $E \subset V \times V $ is the set of edges, and  $\mathbf{A} \in \mathbb{R}^{m \times m}$ is the adjacency matrix, the diagonal degree matrix $\mathbf{D}$ will have elements $\mathbf{D}_{ii} = \sum_j \mathbf{A}_{ij}$. The graph Laplacian matrix is $\mathbf{L} = \mathbf{D} - \mathbf{A}$, which can be normalized as $\mathbf{L} = \mathbf{I}_m - \mathbf{D}^{-\frac{1}{2}}\mathbf{A} \mathbf{D}^{-\frac{1}{2}}$, where $\mathbf{I}_m$ is the identity matrix. As $\mathbf{L}$ is a real symmetric positive semidefinite matrix, it has a set of orthonormal eigenvectors $\{u_l\}_{l=0}^{m-1}\in \mathbb{R}^{m \times m}$, and their associated eigenvalues $\{\lambda_l\}_{l=0}^{m-1}$. The Laplacian is diagonalized by the Fourier basis $[u_0, \cdots,u_{m-1}]\in \mathbb{R}^{m \times m}$ and $\mathbf{L} = \mathbf{U\Lambda U^T}$ where $\mathbf{\Lambda} = diag([\lambda_0,\cdots,\lambda_{m-1}])\in \mathbb{R}^{m\times m}$. The graph Fourier transform of a signal $x\in \mathbb{R}^m$ can then be defined as $\hat{x} = \mathbf{U^T}x \in \mathbb{R}^m$\cite{shuman2013emerging}. The transform enables the convolution operation on graph in the Fourier domain. Suppose a signal vector $\mathbf{x} : V \rightarrow \mathbb{R}$ is defined on the nodes of graph $G$, where $\mathbf{x}_i$ is the value of $\mathbf{x}$ at the $i^{th}$ node. Then the signal $\mathbf{x}$ can be filtered by $g_\theta$ as
% \begin{align}
%     y = g_\theta*\mathbf{x} = g_\theta(\mathbf{L})\mathbf{x} = g_\theta(\mathbf{U{\Lambda}U})\mathbf{x} = \mathbf{U}g_\theta(\Lambda)\mathbf{U^T}\mathbf{x}
% \end{align}
% where the filter $g_\theta(\Lambda)$ can be defined as $g_\theta(\Lambda) = diag(\theta)$ and the parameter $\theta \in \mathbb{R}^n$ is a vector of Fourier coefficients\cite{shuman2013emerging}.

% In \cite{bruna2013spectral}, GCN was formulated for the first time, which was parameterized on the eigenvectors of Laplacian. However, their computations of the eigendecompostition are very expensive, and the filters represented in the spectral domain may not be localized in the graph spatial domain. To overcome these issues, the work in~\cite{defferrard2016convolutional} proposed to use a polynomial filter by
% \vspace{-0.5em}
% \begin{align}
%     g_{\theta}(\Lambda) = \sum_{k=0}^{K-1}{\theta_k}{\Lambda^k}
% \end{align}
% where the parameter $\theta\in {\mathbb{R}}^K$ is a vector of polynomial coefficients. According to \cite{defferrard2016convolutional}, the above filter is exactly $K$-localized, which means the nodes with shortest path length greater than $K$ are not considered for the convolution.
% To further reduce computational complexity, \cite{defferrard2016convolutional} proposed to use the Chebyshev polynomials which can be computed recursively by $T_k(\mathbf{x}) = 2\mathbf{x}T_{k-1}(\mathbf{x}) - T_{k-2}(\mathbf{x})$ with $T_0 = 1$ and $T_1 = \mathbf{x}$, and a filter of order $K-1$ is parameterized as the truncated expansion 
% \vspace{-0.5em}
% \begin{align}
%     g_{\theta}(\Lambda) = \sum_{k=0}^{K-1}{\theta_k}T_k(\hat{\Lambda})
% \end{align}
% Then filtering operation can be written as $y = g_\theta(\mathbf{L})\mathbf{x} = \sum_{k=0}^{K-1}\theta_kT_k(\hat{L})\mathbf{x}$, where $T_k(\hat{L})\in \mathbb{R}^{n\times n}$ is the Chebyshev polynomial of order k with the Laplacian $\hat{L} = 2L/\lambda_{max} - I_n$. The $j^th$ output feature map of sample s is then given by
% \vspace{-0.5em}
% \begin{align}
%     y_{s,j} = \sum_{i=1}^{F_{in}}g\theta_{i,j}(L)x_{s,i}\in \mathbb{R}^m
% \label{eq:filter}
% \end{align}
% where $x_{s,i}$ are the input feature maps, and $F_{in}$ represents the number of input filters. The $F_{in}\times F_{out}$ vectors of Chebyshev coefficients $\theta_{i,j}\in \mathbb{R}^K$ are the layer's trainable parameters. 
%\vspace{-3mm}
\paragraph{\textbf{Higher-order Graph Convolutional Networks.}}
As discussed above, GCN networks use spectral filterings, which consider localized convolutions while ignoring vertices with shortest path length beyond a threshold. This limits the ability of traditional GCNs to learn the complex structural patterns of graphs, such as the community structure, motif patterns, higher-order proximity, etc. Recently, high-order structural patterns were shown to be crucial for learning more accurate graph representations~\cite{ahmed2015efficient,rossi2018higher,benson2016higher,rossi2017deep}. %While it is possible for GCNs to learn these higher-order patterns under certain conditions, for example, stacking more hidden GCN layers to allow more information to flow across the graph. These conditions are unlikely to work well in practice, which is due to the non-linearity of the GCN layers and other factors in the GCN model. 

Thus, we modify the traditional GCN model to operate directly on graphs with higher-order proximity representations so that the higher-order information will be incorporated during the convolutions. Specifically, we employ a random walk sampling process on graphs to obtain the higher-order proximity representations. Random walk sampling has been widely used for learning graph embedding that capture the higher-order proximity and community structure in the graph~\cite{perozzi2014deepwalk,ahmed2018learning}. In our framework, the random walk strategy helps incorporate the higher-order structural information into the graph representations, which further allows for the higher-order graph convolutions in GCNs to capture community and organizational structure of brain networks.% for the similarity learning task.

We denote a random walk rooted at vertex $v_i$ as $W_{v_i}$, which is a stochastic process with random variables $W_{v_i}^1, W_{v_i}^2, \cdots, W_{v_i}^n$, and $W_{v_i}^{j+1}$ is a vertex chosen randomly from the neighbors of vertex $W_{v_j}$. Given a graph $G$, the random walk generator samples uniformly a random vertex $v_i$ as the root of the random walk. The walk uniformly samples a vertex from the neighbors of the root, after which it continues sampling from the neighbors of the last vertex visited until the maximum walk length is reached. There could be multiple walks starting from each vertex, depending on the number of walks specified\cite{perozzi2014deepwalk}. Line $2-9$ in Algorithm \ref{alg:Multihop_SGCN} illustrates the random walk sampling we use for capturing higher-order proximity information. Note that we slide a window with size $w$ on each walk generated and record the frequency of nodes that co-occur within a window in $\mathbf{F}$, and $w$ is a parameter that controls the extent of the higher-order proximity considered in the graph representation. After we obtain the adjacency matrix $\mathbf{A}$ in Line $12$ of Algorithm \ref{alg:Multihop_SGCN} for the higher-order proximity representation, we use $\mathbf{A}$ for computing the Laplacian matrix $\mathbf{L}$, and use this $\mathbf{L}$ for the spectral filtering in Equation (\ref{eq:filter_signal}) to enable the higher-order graph convolutions.
\vspace{-1mm}
\paragraph{\textbf{Algorithm Description.}}
Algorithm \ref{alg:Multihop_SGCN} shows the overall process of the Higher-order Siamese GCN approach. As the spectral graph convolutional networks filter signals are defined on a common graph Laplacian for all samples, we first estimate the mean functional connectivity matrix among the training samples by computing the mean affinity matrix over the graphs and obtain the k-nn graph $\Bar{G}$ using the correlation distance between region pairs. Then we obtain the binary adjacency matrix $\Bar{\mathbf{A}}$ for $\Bar{G}$ as its graph representation. In order to obtain the higher-order proximity representation of the graph, we apply random walk on $\Bar{G}$, after which we slide a window with size $w$ on each walk to get the co-occurrence frequency between two nodes and record the frequency in the matrix $F$. After the random walk sampling stage, we obtain the $k$-nn graph $G'$ based on $F$, where the edges encode the higher-order proximity of the original graph $\Bar{G}$. Then we merge the edges of $G'$ into $\Bar{G}$ to get the updated graph representation with higher-order proximity and obtain the adjacency matrix of the updated graph as $\mathbf{A}$. We compute the Laplacian matrix of the new graph representation and denote it with $\mathbf{L}$. Now we start the model learning of Higher-order Siamese GCN. We first prepare the pairs of training samples from $\mathcal{G}$ with label $Y_{ij} = 1$ for each pair of same class and $Y_{ij} = -1$ for each pair with different classes. We also initialize the neural network parameters $\Theta$ of the GCNs with Siamese network. Then we input the pairs into the Siamese GCNs and perform spectral convolutions according to Equation (\ref{eq:filter}). Specifically, for each input brain network, we use the functional correlation value of node $v_s$ with $v_i$ as the signal $x_{s,i}$ in Equation (\ref{eq:filter}). After the convolutions, the outputs of the twin GCNs are then combined by a dot product layer, followed by a fully connected (FC) layer that integrates the information learned from the preceding filters and output a similarity estimiate $s_{ij}$ for the input pair $G_i$ and $G_j$. Then we compute the loss for the Siamese network. We use the Hinge loss in Equation (\ref{hinge_loss}), by minimizing which the mean similarity between input pairs belonging to the same class will be maximized while the mean similarity between pairs belonging to different classes will be minimized.   We use stochastic gradient descent with Adaptive Moment Estimation (ADAM) optimizer to train the model.
\vspace{-0.3em}
\begin{align}
    L^{hinge} = \frac{1}{N_p}\sum_{i=1}^{N}\sum_{j=i+1}^{N} max(0,1-{Y_{ij}}{s_{ij}}),
    \label{hinge_loss}
\end{align}
where $N$ is the total number of subjects in the training set, and $N_p = N(N-1)/2$ is the total number of pairs from the training set.
%To optimize the model, we apply the stochastic gradient descent with Adaptive Moment Estimation (ADAM) algorithm proposed in \cite{kingma2014adam}. After the training process, we will have a well trained Higher-order Siamese GCN model for learning similarity scores between a pair of brain networks.
% \begin{align}
%     L^{hinge} = \frac{1}{N}\sum_{i=0}^{N-1}max(0,1-{y_i}{s_i}),
%     \label{hinge_loss}
% \end{align}

\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
% \begin{minipage}{.7\linewidth}
\begin{algorithm}[t]
\caption{Higher-order Siamese GCN}
\label{alg:Multihop_SGCN}
\begin{algorithmic}[1] 
\scriptsize
\Require $\mathcal{G} = {G_1, G_2, \cdots, G_n}$ (training graph samples); $\mathbf{y}$(class labels); random walk parameters: $\gamma$ (number of walks), $l$ (walk length), $w$ (window size)\\
%\Ensure $\Theta$\\
    Obtain the mean $k$-nn graph $\Bar{G}(V,E,\Bar{\mathbf{A}})$;\\
    Initialize a frequency matrix $\mathbf{F}\in \mathbb{R}^{m\times m}$ with $0$s;
    \For {$i = 0$ to $\gamma$}
    \State $V'=$ Shuffle$(V)$;
    \For{\textbf{each} $v_i \in V'$}
    \State $W_{v_i} = RandomWalk(\Bar{G},v_i,l)$;
    % \For{\textbf{each} $v_j \in W_{v_i}$}
    % \For{\textbf{each} $u_k \in W_{v_i}[j - w : j + w]$}
    % \State $\mathbf{F}_{{v_j},{u_k}} += 1$
    % \State $\mathbf{F}_{{u_k},{v_j}} += 1$
    % \EndFor
    % \EndFor
    \State Update $\mathbf{F}$;
    \EndFor
    \EndFor\\
    % Obtain the $k$-nn graph from $\mathbf{F}$, with its adjacency matrix $\mathbf{A}$; \\
    % Compute the Laplacian matrix $L$; \\
    Obtain a $k$-nn graph $G'$ based on $\mathbf{F}$;\\
    Merge the edges of $G'$ into $\Bar{G}$; \\
    Obtain the updated adjacency matrix $\mathbf{A}$;\\
    Prepare pairs of training samples from $\mathcal{G}$;\\
    Initialize the parameters $\Theta$ of GCNs in Siamese network;
    \While {not converge}
    \State Perform spectral filterings according to Equation (\ref{eq:filter}); 
    \State Compute the similarity estimate $s_{ij}$ for the input pair $(G_i,G_j)$;
    \State Compute the loss $L^{hinge}$ according to Equation (\ref{hinge_loss}) ;
    \State Apply stochastic gradient descent with ADAM optimizer to update $\Theta$;
    \EndWhile
\end{algorithmic}
\end{algorithm}
% \end{minipage}
%loss functions for the regression model
% \begin{align}
%   L_R = \sum _{i=1}^{n}||g(f(G_i)) - y_i||_2^2  
% \end{align}

% \begin{align}
%     L_F = \sum _{i=1}^{K}||f(X_{i,1}) -f(X_{i,2})||_2^2 - ||y_{i,1}-y_{i,2}||_2^2
% \end{align}

% \begin{align}
%     L = L_R + L_F + \lambda ||w||_2^2
% \end{align}
\vspace{-0.1em}

%This is the old version of preliminaries and framework
\begin{comment}
\section{Preliminaries}

\textcolor{red}{\textbf{TODO}: this discussion (next two paragraphs) is too long so shrink it, some of this could be moved to the intro/related work}

In many machine learning problems where data comes in graphs, a key application is how to measure the similarity between graphs. In the field of brain network analysis, measuring similarity between brain networks is especially important for further analysis such as brain disorder diagnosis. Existing methods for similarity estimation between graphs are mainly based on graph embedding, graph kernels or motifs \cite{livi2013graph}. These methods are designed for specific scenarios and have their limitations. For example, the graph embedding learned in \cite{abraham2017deriving} may discard structural information that could be important for similarity estimation. In \cite{takerkart2014graph}, the graph kernels used for brain network comparison focus on features of small subgraphs, which ignored global structures of graph. Another problem in these works is that the graph feature extraction and similarity estimation are done in completely separate stages, where the features extracted may not be suitable for similarity estimation. 

Recently, a metric learning method with spectral graph convolutions is proposed in \cite{ktena2018metric}, where a Siamese network with graph convolutional neural networks is used to get similarity estimate of two brain connectivity networks. This method consists of two components: (a) Graph Convolutional Network(GCN) and (b) Siamese Network. This method shows promising results in the experiment of similarity estimate between brain connectivity networks. However, the way that GCN was used in that work focuses on local structure in the graph representation, while ignoring high-order structural information, which makes the method less generic. %especially for large graphs. 
In this paper, we go beyond of that method and propose a Higher-order Siamese GCN approach, which is a general framework with different options in each component, and the Multi-hop property of the approach allows us to incorporate high-order structural information from the graph representations into the learning process. In this section, we will first introduce GCN and Siamese network individually. Then we will introduce the proposed Higher-order Siamese GCN approach, which is a general framework with different options in each component for similarity learning of graphs.

\subsection{Graph Convolutional Networks}
Graph convolutional network (GCN), as a generalized convolutional neural network from grid-structure domain to graph-structure domain, has been emerging as a powerful approach for graph mining \cite{bruna2013spectral,defferrard2016convolutional}. In GCNs, filters are defined in the graph spectral domain. Given a graph $G=(V, E, \mathbf{A})$, where $V$ is the set of vertices, $E \subset V \times V $ is the set of edges, and  $\mathbf{A} \in \mathbb{R}^{m \times m}$ is the adjacency matrix, the diagonal degree matrix $\mathbf{D}$ will have elements $\mathbf{D}_{ii} = \sum_j \mathbf{A}_{ij}$. The graph Laplacian matrix is $\mathbf{L} = \mathbf{D} - \mathbf{A}$, which can be normalized as $\mathbf{L} = \mathbf{I}_m - \mathbf{D}^{-\frac{1}{2}}\mathbf{A} \mathbf{D}^{-\frac{1}{2}}$, where $\mathbf{I}_m$ is the identity matrix. As $\mathbf{L}$ is a real symmetric positive semidefinite matrix, it has a set of orthonormal eigenvectors $\{u_l\}_{l=0}^{m-1}\in \mathbb{R}^{m \times m}$, and their associated eigenvalues $\{\lambda_l\}_{l=0}^{m-1}$. The Laplacian is diagonalized by the Fourier basis $[u_0, \cdots,u_{m-1}]\in \mathbb{R}^{m \times m}$ and $\mathbf{L} = \mathbf{U\Lambda U^T}$ where $\mathbf{\Lambda} = diag([\lambda_0,\cdots,\lambda_{m-1}])\in \mathbb{R}^{m\times m}$. The graph Fourier transform of a signal $x\in \mathbb{R}^m$ can then be defined as $\hat{x} = \mathbf{U^T}x \in \mathbb{R}^m$\cite{shuman2013emerging}. The transform enables the convolution operation on graph in the Fourier domain. Suppose a signal vector $\mathbf{x} : V \rightarrow \mathbb{R}$ is defined on the nodes of graph $G$, where $\mathbf{x}_i$ is the value of $\mathbf{x}$ at the $i^{th}$ node. Then the signal $\mathbf{x}$ can be filtered by $g_\theta$ as
\begin{align}
    y = g_\theta*\mathbf{x} = g_\theta(\mathbf{L})\mathbf{x} = g_\theta(\mathbf{U{\Lambda}U})\mathbf{x} = \mathbf{U}g_\theta(\Lambda)\mathbf{U^T}\mathbf{x}
\end{align}
where the filter $g_\theta(\Lambda)$ can be defined as $g_\theta(\Lambda) = diag(\theta)$ and the parameter $\theta \in \mathbb{R}^n$ is a vector of Fourier coefficients\cite{shuman2013emerging}.

In \cite{bruna2013spectral}, GCN was formulated for the first time, which was parameterised on the eigenvectors of Laplacian. However, their computations of the eigendecompostition are very expensive, and the filters represented in the spectral domain may not be localized in the graph spatial domain. To overcome these issues, \cite{defferrard2016convolutional} proposed to use a polynomial filter by
\begin{align}
    g_{\theta}(\Lambda) = \sum_{k=0}^{K-1}{\theta_k}{\Lambda^k}
\end{align}
where the parameter $\theta\in {\mathbb{R}}^K$ is a vector of polynomial coefficients. According to \cite{defferrard2016convolutional}, the above filter is exactly $K$-localized, which means the nodes with shortest path length greater than $K$ are not considered for the convolution.
To further reduce computational complexity, \cite{defferrard2016convolutional} proposed to use the Chebyshev polynomials which can be computed recursively by $T_k(\mathbf{x}) = 2\mathbf{x}T_{k-1}(\mathbf{x}) - T_{k-2}(\mathbf{x})$ with $T_0 = 1$ and $T_1 = \mathbf{x}$, and a filter of order $K-1$ is parameterized as the truncated expansion 
\begin{align}
    g_{\theta}(\Lambda) = \sum_{k=0}^{K-1}{\theta_k}T_k(\hat{\Lambda})
\end{align}
Then filtering operation can be written as $y = g_\theta(\mathbf{L})\mathbf{x} = \sum_{k=0}^{K-1}\theta_kT_k(\hat{L})\mathbf{x}$, where $T_k(\hat{L})\in \mathbb{R}^{n\times n}$ is the Chebyshev polynomial of order k with the Laplacian $\hat{L} = 2L/\lambda_{max} - I_n$. The $j^th$ output feature map of sample s is then given by
\begin{align}
    y_{s,j} = \sum_{i=1}^{F_{in}}g\theta_{i,j}(L)x_{s,i}\in \mathbb{R}^m
\label{eq:filter}
\end{align}
where $x_{s,i}$ are the input feature maps, and $F_{in}$ represents the number of input filters. The $F_{in}\times F_{out}$ vectors of Chebyshev coefficients $\theta_{i,j}\in \mathbb{R}^K$ are the layer's trainable parameters. A graph convolutional neural network can therefore be built by stacking multiple convolutional layers in the form of Eq.~\ref{eq:filter}, with a non-linearity following each layer. 

\subsection{Siamese Network}
Siamese networks were first introduced in \cite{bromley1994signature} to solve image matching problem for signature verification. A Siamese network consists of two twin neural networks who share parameters with each other. The inputs of the twin networks are distinct, but their highest-level feature representations are joined by a function at the top. As the parameters between the twin networks are tied, each input will be processed in the same way respectively in the twin networks, which can guarantee that similar input samples not be mapped to very different locations by the respective networks. Therefore, the Siamese network tend to be good for differentiating the two inputs or measuring the similarity between them. Some existing works on image similarity learning use CNNs in the twin networks of Siamese, as CNNs works well in learning 2D grid features from images\cite{chopra2005learning}. In this work, as we aim to learn similarity metric between graphs, we explore the capability of GCNs with Siamese architecture. Fig.~\ref{fig:siamese} shows a simple illustration of the Siamese architecture with GCNs in the twin networks.

\subsection{Higher-order Siamese GCN: A General Framework}
As introduced above, GCN uses spectral filterings, which consider localized convolutions while ignoring the nodes with shortest path length beyond a threshold. However, high-order structural information are very important for learning from graphs \cite{rossi2018higher,benson2016higher,rossi2017deep}. In this section, we introduce a general framework for similarity learning of graphs, which is able to capture high-order structure of graphs and incorporate it into the similarity learning process. Fig.~\ref{fig:framework} shows the framework we propose. The detailed illustration of the proposed framework is as follows.
\paragraph{\textbf{Problem Definition.}}
Given a pair of graphs $G_i=(V_i, E_i, \mathbf{A_i})$ and $G_j=(V_j, E_j, \mathbf{A_j})$, where $V_i$ and $V_j$ contain the same number of vertices with fully aligned physical meanings, the goal of similarity learning on the pair of graphs is to learn a similarity score $s$ between $G_i$ and $G_j$. 

\paragraph{\textbf{Random Walk Sampling.}}
Random walk, as a way for sampling, has been used for sampling vertexes or edges for graphs, and the sampling on graphs tend to capture community structure information\cite{perozzi2014deepwalk,ahmed2018learning}. In this paper, we employ a random walk sampling process on graphs and aim to refine the graph representations with the high-order structural information obtained by the random walks, which will be further incorporated into the similarity learning process in the framework. 
We denote a random walk rooted at vertex $v_i$ as $W_{v_i}$, which is a stochastic process with random variables $W_{v_i}^1, W_{v_i}^2, \cdots, W_{v_i}^k$, and $W_{v_i}^{j+1}$ is a vertex chosen randomly from the neighbors of vertex $W_{v_j}$. Given a graph $G$, the random walk generator samples uniformly a random vertex $v_i$ as the root of the random walk. The walk uniformly samples a vertex from the neighbors of the root, after which it continues sampling from the neighbors of the last vertex visited until the maximum path length is reached. There could be multiple walks starting from each vertex, depending on the number of walks specified\cite{perozzi2014deepwalk}. Line $2-14$ in Algorithm \ref{alg:Multihop_SGCN} illustrates the random walk sampling process we employ for capturing high-order structure information. Note that we slide a window with size $w$ on each walk generated and record the frequency of nodes that cooccur within a window in $\mathbf{F}$, and $w$ decides the number of hops considered for refining the graph representation. 

\begin{figure}[t]
    \centering
    \includegraphics[width = 0.55 \columnwidth]{Figure1_Siamese.png}
    \caption{Siamese Architecture with Graph Convolutional Networks}
    \label{fig:siamese}
\end{figure}

\paragraph{\textbf{Higher-order Siamese GCN.}}

Algorithm \ref{alg:Multihop_SGCN} shows the overall process of the Higher-order Siamese GCN approach. As the spectral graph convolutional networks filter signals are defined on a common graph structure for all samples, we first estimate the mean functional connectivity matrix among the training samples by computing the mean adjacency matrix $\Bar{\mathbf{A}}$ over the graphs and obtain the average graph $\Bar{G}$. In order to refine the graph representation, we apply random walk on $\Bar{G}$, after which we slide a window with size $w$ on each walk to get the cooccurrence frequency between two nodes and record the frequency in the matrix $F$. After the random walk sampling stage, we obtain a $k$-nn graph, which is the refined graph encoded with high-order structure of the original graph. We compute the Laplacian matrix of the refined graph and denote it with $\mathbf{L}$. Now we start the model learning of Higher-order Siamese GCN. We first prepare the pairs of training samples from $D$ with label $1$ for each pair of same class and $0$ for each pair with different classes. We also initialize the neural network parameters $\Theta$ of the GCNs with Siamese network. Then we input the pairs into the Siamese GCNs and perform spectral convolutions, after which the outputs of the twin GCNs are combined and a similarity estimiate $s_i$ will be obtained for each $i^{th}$ pair. Then we compute the loss for the Siamese network. We use the Hinge loss in Equation (\ref{hinge_loss}). To optimize the model, we apply the stochastic gradient descent with Adaptive Moment Estimation (ADAM) algorithm proposed in \cite{kingma2014adam}. After the training process, we will have a well trained Higher-order Siamese GCN model for learning similarity scores between a pair of graphs.

\begin{align}
    L^{hinge} = \frac{1}{N}\sum_{i=0}^{N-1}max(0,1-{y_i}{s_i}),
    \label{hinge_loss}
\end{align}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}
\begin{algorithm}[t]
\caption{High-order Siamese GCN}
\label{alg:Multihop_SGCN}
\begin{algorithmic}[1] 
\small
\Require $D={G_1, G_2, \cdots, G_n}$ (training graph samples); $\mathbf{y}$(class labels); random walk parameters: $\gamma$ (number of walks), $l$ (walk length), $w$ (window size)\\
%\Ensure $\Theta$\\
    Compute $\Bar{\mathbf{A}}$ for $\Bar{G}(V,E)$;\\
    Initialize a frequency matrix $\mathbf{F}\in \mathbb{R}^{m\times m}$ with $0$s;
    \For {$i = 0$ to $\gamma$}
    \State $V'=$ Shuffle$(V)$;
    \For{\textbf{each} $v_i \in V'$}
    \State $W_{v_i} = RandomWalk(\Bar{G},v_i,l)$;
    % \For{\textbf{each} $v_j \in W_{v_i}$}
    % \For{\textbf{each} $u_k \in W_{v_i}[j - w : j + w]$}
    % \State $\mathbf{F}_{{v_j},{u_k}} += 1$
    % \State $\mathbf{F}_{{u_k},{v_j}} += 1$
    % \EndFor
    % \EndFor
    \State Update $\mathbf{F}$;
    \EndFor
    \EndFor\\
    % Obtain the $k$-nn graph from $\mathbf{F}$, with its adjacency matrix $\mathbf{A}$; \\
    % Compute the Laplacian matrix $L$; \\
    Obtain a $k$-nn graph based on $\mathbf{F}$;\\
    Add the edges of the $k$-nn graph into $\Bar{G}$; \\
    Obtain the refined adjacency matrix $\mathbf{A}$;\\
    Prepare pairs of training samples from $D$;\\
    Initialize the parameters $\Theta$ of GCNs in Siamese network;
    \While {not converge}
    \State Perform spectral filterings according to Equation (\ref{eq:filter}); 
    \State Compute the similarity estimate $s_i$ for the $i^{th}$ pair;
    \State Compute the loss $L^{hinge}$ according to Equation (\ref{hinge_loss}) ;
    \State Apply stochastic gradient descent with ADAM optimizer to update $\Theta$;
    \EndWhile
\end{algorithmic}
\end{algorithm}
%loss functions for the regression model
% \begin{align}
%   L_R = \sum _{i=1}^{n}||g(f(G_i)) - y_i||_2^2  
% \end{align}

% \begin{align}
%     L_F = \sum _{i=1}^{K}||f(X_{i,1}) -f(X_{i,2})||_2^2 - ||y_{i,1}-y_{i,2}||_2^2
% \end{align}

% \begin{align}
%     L = L_R + L_F + \lambda ||w||_2^2
% \end{align}
\vspace{-0.1em}
\end{comment}

==> sec_intro.tex <==
%%%%%%%%% BODY TEXT
\section{Introduction}
\label{sec:intro}
%\textbf{\textcolor{red}{Nesreen: cite more references for the similarity learning problem}}

Learning a similarity metric has gained much attention recently in a variety of real-world applications, where the goal is to learn a function that maps input patterns to a target space while preserving the semantic distance in the input space~\cite{wang2014learning,chopra2005learning,guo2001learning,chechik2009online,bautista2017deep}. For example, finding images that are similar to a query image is an indispensable problem in search engines \cite{wang2014learning}, and an effective image similarity metric is the key for finding similar images. Similarity learning is particularly suitable for applications where the number of classes is very large, the number of samples is very small, and/or only a subset of classes is known at the time of training (e.g., face recognition applications). Metric learning systems are typically trained on pairs of patterns from the training set (e.g., pairs of images, graphs, etc), with the goal to find a function that maps the input patterns to a target space such that the distance among patterns in the target space approximates the semantic distance in the input space. Given a family of possible models (functions) with parameter weights $\mathbb{W}$, the goal is to find the value of optimal weights $\mathbb{W}$, such that the estimated similarity score of the input pair $(X_1, X_2)$ is small if $X_1$ and $X_2$ belong to the same class, and large if they belong to different classes. The loss function used in training maximizes the mean similarity between input pairs belonging to the same class, and minimizes the mean similarity between pairs belonging to different classes.   

%In \cite{bautista2017deep}, similarity learning is formulated as a partial ordering task with soft correspondences of all samples to classes. Adopting a strategy of self-supervision, a CNN is trained to optimally represent samples in a mutually consistent manner while updating the classes. The similarity learning and grouping procedure are integrated in a single model and optimized jointly. Another deep learning model for ranking was proposed in \cite{wang2014learning} for learning fine-grained image similarity. An efficient triplet sampling algorithm is proposed to learn the model with distributed asynchronous stochastic gradient. The proposed approach is shown to outperform models based on hand-crafted visual features and deep classification models. 

While  the majority of the similarity learning research is focused on images, our work focused instead on learning a similarity metric for neuroimages, such as fMRI images and DTI images. Functional magnetic resonance imaging (fMRI) measures brain activity by detecting changes associated with blood flow, and has been widely used in cognitive neuroscience, medical, and clinical applications. We particularly focus on brain connectivity networks (i.e., functional networks) extracted from the input fMRI images, where the observed brain activity is modeled as a network of inter-regional functional associations. The resulting functional networks can be analyzed/modeled using graph-theoretic and graph machine learning techniques. The analysis of brain connectivity networks has revealed many key features of the brain organization, such as the modular structure of the brain, and the presence of hubs~\cite{bertolero2015modular,power2011functional}.   

%\textbf{\textcolor{red}{Nesreen: this paragraph is difficult to read and does not sound scientifically correct, needs fixing.
%Existing works in this area have shown that the structural information in human brain networks reflect brain activity patterns, and people with brain disorders tend to have different patterns with healthy people \cite{ma2016multi,ma2017multib}. Thus, the graph representation provides significant advantages in capturing the structure information of the human brain. Therefore, we study the similarity learning problem in the graph structure domain and aim to apply it for fMRI brain connectivity (network) analysis.}}  

Graph convolutional neural networks (GCNs) have emerged to learn deep representations of graph-structured data, %Graph convolutional neural networks have been applied on graphs to learn embedding for node classification or other relevant tasks 
and been shown to outperform other traditional relational learning methods~\cite{defferrard2016convolutional,li2018deeper}. However, these works focus mainly on social and information networks, to model the node/graph similarity, where the relationships/links are usually given or well-defined (e.g., friendship, retweet, following links). In this paper, however, we focus on learning deep representations from fMRI brain connectivity networks, where each brain network represents the brain activity patterns of a particular subject. Brain connectivity networks are widely used to model inter-regional functional connections, and are typically inferred from the input fMRI data of each subject. Each brain connectivity network is usually represented by a graph constructed from input fMRI data where the nodes represent brain regions and the edges represent the pairwise region-to-region correlations. However, the organization of brain connectivity networks is constrained by various factors, such as the underlying brain anatomical network~\cite{hagmann2008mapping,honey2009predicting}, which has an important contribution in shaping the activity across the brain. These constraints pose significant challenges on characterizing the structure and organization of brain connectivity networks. In addition, these constraints lead to distance-dependent inter-regional correlations, where activity patterns from nearby brain regions is strongly correlated due to spatial factors than the activity from distant ones. Thus, it's crucial to distinguish between long-range functional connectivity that represents the brain inter-regional communications, which arise from functional necessity, from those that arise due to spatial constraints~\cite{honey2009predicting}. We propose an end-to-end similarity learning framework for multi-subject fMRI data. The proposed framework learns the brain network representations via a supervised metric-based approach with siamese neural networks and using two GCNs as the twin networks. Our proposed framework performs higher-order convolutions by incorporating higher-order proximity via random walks in graph convolutional networks. We use this approach to characterize the community and organizational structure in brain connectivity networks, and to emphasize the contribution of the long-range functional connectivity. To the best of our knowledge, this is the first community-preserving similarity learning framework for multi-subject brain network analysis. 

The principle aim of this work is to build a framework that can learn discriminative structural features of brain connectivity networks for multi-subject analysis. However, the complex structure of these networks poses significant challenges to such a framework. For example, prior work has shown the importance of higher-order proximity structure such as the community structure of brain networks in health as well as neuropsychiatric disorders~\cite{ma2016multi,ma2017multi}. However, current graph neural methods are capable of only learning local neighborhood information and cannot directly capture the higher-order proximity and community structure of graphs. Although it might be possible for GCNs to learn these higher-order patterns under certain conditions, for example, stacking more hidden GCN layers to allow more information to flow across the graph, these conditions are unlikely to work well in practice, which is due to the non-linearity of the GCN layers, and the difficulty of fitting the larger number of parameters with a limited number of training samples (e.g., the limited samples in neuroimaging data) which leads to overfitting (see Figures~\ref{fig:acc_K} and~\ref{fig:acc_Layers}). Thus, how to generalize GCNs to capture the community structure of brain networks is a key challenge. Moreover, how to leverage the structural features learned by GCNs for similarity learning and build an end-to-end similarity learning framework for multi-subject analysis is another challenging problem. Our proposed framework leverages higher-order graph convolutional networks to characterize the community and organizational structure of brain connectivity networks. We conjecture this framework would be useful for the multi-subject brain analysis in health and neuropsychiatric disorders~\cite{greicius2008resting}. Our main contributions are summarized as follows:
%Due to the sophisticated structures and specific properties of brain networks, it is very challenging to build a framework that can learn discriminating graph structure features from brain networks using GCNs for multi-subject analysis. To begin with, previous study has shown that higher-order information such as the community structure in brain networks are very important for discriminating neurological disorders and normal controls \cite{ma2016multi,ma2017multi}. However, the original GCNs focus on learning localized neighborhood information and can not directly capture the higher-order information of graphs \cite{defferrard2016convolutional}. Although it might be possible for GCNs to learn these higher-order patterns under certain conditions, for example, stacking more hidden GCN layers to allow more information to flow across the graph, these conditions are unlikely to work well in practice, which is due to the non-linearity of the GCN layers and the difficulty of tuning the larger number of parameters with a limited number of training samples which is a usual case for neuroimaging data. Therefore, how to generalize the original GCNs so that it can capture both localized neighborhood information and higher-order information for brain network analysis is a key challenge. Moreover, how to leverage the graph structure information learned by GCNs for similarity learning and build an end-to-end similarity learning framework to facilitate the further multi-subject neurological and cognitive status analysis is also a challenging problem. 
%Due to the sophisticated structures and specific properties of brain networks, it is very challenging to build a framework that can learn discriminating graph structure features from brain networks using GCNs for multi-subject analysis. To begin with, previous study has shown that higher-order information such as the community structure in brain networks are very important for discriminating neurological disorders and normal controls \cite{ma2016multi,ma2017multi}. However, the original GCNs focus on learning localized neighborhood information and can not directly capture the higher-order information of graphs \cite{defferrard2016convolutional}. Although it might be possible for GCNs to learn these higher-order patterns under certain conditions, for example, stacking more hidden GCN layers to allow more information to flow across the graph, these conditions are unlikely to work well in practice, which is due to the non-linearity of the GCN layers and the difficulty of tuning the larger number of parameters with a limited number of training samples which is a usual case for neuroimaging data. Therefore, how to generalize the original GCNs so that it can capture both localized neighborhood information and higher-order information for brain network analysis is a key challenge. Moreover, how to leverage the graph structure information learned by GCNs for similarity learning and build an end-to-end similarity learning framework to facilitate the further multi-subject neurological and cognitive status analysis is also a challenging problem. 
%In this paper, we propose the higher-order graph convolutions, which can capture both the localized neighborhood information and higher-order structural information of graphs. We incorporate the graph information learned by the higher-order GCNs into the similarity learning of graphs with the Siamese network. Specifically, we apply a random walk strategy with sliding windows to capture higher-order structure information in graphs and incorporate the higher-order structure information into the graph representations in GCNs, which eventually allows for higher-order convolutions on graphs. 
%Our main contributions can be summarized as follows:
% Since there are various structure information in graphs and the brain networks might differ in global structure or local structure, the main challenge of this similarity learning task is in how to build a general learning framework that can learn discriminating graph structure features from graphs using GCNs and leverage the graph structure for the similarity learning task. Recently, \cite{ktena2018metric} studied the similarity learning problem on graphs with GCNs and applied to fMRI brain networks, which is the most relevant work to our work in this paper. However, they did not consider high-order information of graphs when applying GCNs, thus may ignore important graph features in the similarity learning process. In this paper, we propose to incorporate the high-order structural information of graphs into the GCNs, and build a framework with Siamese network for similarity learning of graphs. Specifically, we apply a random walk strategy with sliding windows to capture high-order information on graphs and use it to refine the graph representations, which allows for higher-order convolutions on graphs. Our contributions can be summarized as follows: 
\begin{itemize}
\setlength{\itemsep}{0pt}
    \item We propose an end-to-end similarity learning framework called "Higher-order Siamese GCN" for metric learning of graph data. The framewrok learns the brain network representations via a supervised metric-based approach with siamese neural networks and using two GCNs as the twin networks. The framework leverages higher-order graph convolutions to characterize the community structure of brain connectivity networks.

    \item We apply the proposed framework on four real fMRI brain network datasets for similarity learning with respect to brain health status and cognitive abilities. The experiment results demonstrate the effectiveness and advantage of the proposed framework for neurological disorder analysis with respect to three kinds of disease (i.e., Autism, Bipolar and HIV) and the cognitive analysis for the Human Connectome Project. 
    
    \item Our proposed approach achieves an average AUC gain of $75$\% compared to PCA, $65.5$\% compared to Spectral Embedding, and $24.3$\% compared to S-GCN across a variety of datasets, indicating its promising use cases for multi-subject brain analysis in health and neuropsychiatric disorders.
\end{itemize}
\vspace{-2mm}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width = 0.65 \columnwidth]{brain_voxels.eps}
%     \caption{Example of fMRI image \cite{ma2016spatio}}
%     \label{fig:brain}
% \end{figure}

